DFlow: Diverse Dialogue Flow Simulation with Large Language Models

Developing language model-based dialogue agents requires effective data to train models that can follow specific task logic. However, most existing data simulation methods focus on increasing diversity in language, topics, or dialogue acts at the utterance level, largely neglecting a critical aspect of task logic diversity at the dialogue level. This paper proposes a novel data simulation method designed to enhance the diversity of synthetic dialogues by focusing on task execution logic. Our method uses LLMs to generate decision tree-structured task plans, which enables the derivation of diverse dialogue trajectories for a given task. Each trajectory, referred to as a "dialog flow", guides the generation of a multi-turn dialogue that follows a unique trajectory. We apply this method to generate a task-oriented dialogue dataset comprising 3,886 dialogue flows across 15 different domains. We validate the effectiveness of this dataset using the next action prediction task, where models fine-tuned on our dataset outperform strong baselines, including GPT-4. Upon acceptance of this paper, we plan to release the code and data publicly.

==> 83-extra-figure.tex <==
\begin{figure}[th]
    \centering
    \includegraphics[width=4.cm]{img/flow_diversity.jpg}
    \caption{Flow type distribution of \dataset.}
    \label{fig:flow_type_distribution}
    \vspace{2mm}
\end{figure}

\begin{figure}[th]
    \centering
    \includegraphics[width=8.cm]{img/gpt_longterm_rental_18_flows.png}
    \caption{Sankey diagram showing 18 dialogue flows from "Long-term car rental" plan generated by GPT-3.5-turbo. The height of a node shows the number of flows passing through the node.}
    \label{fig:gpt_flows}
    \vspace{2mm}
\end{figure}




==> tab/ast_ablation.tex <==
\begin{table*}[th]
    \centering
    \small
    \begin{tabular}{llrrrr}
    \toprule
    \textbf{Model} & \textbf{Training Data} & \textbf{Data Size} & \textbf{B-Slot} & \textbf{Value} & \textbf{Joint Accuracy} \\
    \midrule
    RoBERTa-large & ABCD (100\%) & 29K & 93.60\% & 67.20\% & 65.80\% \\
    T5-small  & ABCD (100\%) & 29K & 89.10\% & 89.20\% & 87.90\% \\
    \midrule
    \multirow{3}{*}{OpenLLama-7B-instruct} & ABCD (1\%) & 290 & 43.36\% & 58.31\% & \colorbox{gray!25}{41.20\%} \\
     & ABCD (1\%) + GPT-3.5-turbo & 5,098 & 80.56\% & 86.50\% & \colorbox{green!45}{79.40\%} \\
     & ABCD (1\%) + GPT-3.5-turbo (w.o. plan) & 6,446 & 54.32\% & 66.61\% & \colorbox{red!15}{52.82\%} \\
    \midrule
    \multirow{3}{*}{Falcon-7B-instruct} & ABCD (1\%) & 290 & 11.96\% & 48.50\% & \colorbox{gray!25}{10.47\%} \\
     & ABCD (1\%) + GPT-3.5-turbo & 5,098 & 57.48\% & 72.59\% & \colorbox{green!15}{54.65\%} \\
     & ABCD (1\%) + GPT-3.5-turbo (w.o. plan) & 6,446 & 28.57\% & 54.82\% & \colorbox{red!15}{27.08\%} \\
    \bottomrule
    \end{tabular}
    \caption{Ablation study in the action state tracking task, where we directly prompt GPT-3.5-turbo to generate 10 different dialogues without task plan and flow, and only 1\% ABCD training data are used during the fine-tuning of OpenLLama-7B-instruct and Falcon-7B-instruct.}
    \label{tab:ast_ablation}
\end{table*}

==> tab/ast_data_format.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{p{0.93\linewidth}}
    \toprule
     % \multicolumn{1}{l}{\textbf{The Instruction Tuning Data Format for the Action State Tracking Task}} \\
     % \midrule
     \textbf{Instruction}: Given the full task plan, task flow and dialogue context, predict the current system action. 
     [plan] $p_1, ..., p_n$
     [schema] $a_1[v_1^1, v_1^2, ...], ..., a_m[v_m^1, v_m^2, ...]$ \\
     \midrule
     \textbf{Input}: 
     [context] $u_1, ..., u_{t-1}$
     [flow] $a_1[v_1^1], ..., a_m[v_m^1]$ \\
     \midrule
     \textbf{Output}:  
     [system] $a_t[v_t^1, ..., v_t^n]$ \\ 
    \bottomrule
    \end{tabular}
    \caption{The instruction-tuning data format for the next action prediction task.
    \label{tab:ast_data_format}}
    \vspace{2mm}
\end{table}

==> tab/ast_full.tex <==
\begin{table*}[th]
    \centering
    \small
    \begin{tabular}{llrrrr}
    \toprule
    \textbf{Model} & \textbf{Training Data} & \textbf{Data Size} & \textbf{B-Slot} & \textbf{Value} & \textbf{Joint Accuracy} \\
    \midrule
    RoBERTa-large & ABCD (100\%) & 29K & 93.60\% & 67.20\% & 65.80\% \\
    T5-small & ABCD (100\%) & 29K & 89.10\% & 89.20\% & 87.90\% \\
    \midrule
    \multirow{5}{*}{OpenLLama-7B-instruct} & ABCD (1\%) & 290 & 43.36\% & 58.31\% & \colorbox{gray!25}{41.20\%} \\
     & ABCD (1\%) + GPT-3.5-turbo & 5,098 & 80.56\% & 86.50\% & \colorbox{green!45}{79.40\%} \\
     & ABCD (1\%) + Falcon-40B-instruct & 5,856 & 60.96\% & 75.42\% & \colorbox{green!15}{60.13\%} \\
     & ABCD (1\%) + MPT-30B-chat & 5,487 & 76.25\% & 82.89\% & \colorbox{green!30}{74.75\%} \\
     & ABCD (1\%) + ChatGLM-6B & 3,163 & 54.98\% & 71.10\% & \colorbox{green!10}{54.32\%} \\
    \midrule
    \multirow{5}{*}{Falcon-7B-instruct} & ABCD (1\%) & 290 & 11.96\% & 48.50\% & \colorbox{gray!25}{10.47\%} \\
     & ABCD (1\%) + GPT-3.5-turbo & 5,098 & 57.48\% & 72.59\% & \colorbox{green!15}{54.65\%} \\
     & ABCD (1\%) + Falcon-40B-instruct & 5,856 & 66.45\% & 80.23\% & \colorbox{green!25}{65.61\%} \\
     & ABCD (1\%) + MPT-30B-chat & 5,487 & 39.04\% & 59.80\% & \colorbox{green!5}{37.71\%} \\
     & ABCD (1\%) + ChatGLM-6B & 3,163 & 43.02\% & 62.79\% & \colorbox{green!10}{42.19\%} \\
    \bottomrule
    \end{tabular}
    \caption{Improved model performance using our  simulation datasets in the action state tracking task, where only 1\% ABCD training data are used during the fine-tuning of OpenLLama-7B-instruct and Falcon-7B-instruct.}
    \label{tab:ast_full}
\end{table*}

==> tab/data_compare.tex <==
% \begin{table}[t]
%     \centering
%     \small
%     \begin{tabular}{l|cccc}
%     \toprule
%       &\textbf{MultiWOZ} & \textbf{STAR} & \textbf{ABCD} & \textbf{DialogFlow} \\
%     \midrule
%     % \# Domains & 7 & 13 & 30 & 15 \\
%     % \# Dialogues & 8,438 & 5,820 & 8,034 & 3,876 \\
%     % \# Turns & 115K & 127K & 177K & 35K \\
%     % Avg. Flow Steps & - & - & 3.73 & 7.76 \\
%     % \midrule
%     Task Plan? & \xmark & \xmark & \cmark & \cmark \\
%     Dialogue Flow? & \xmark & \cmark & \cmark & \cmark \\
%     Error Handling? & \xmark & \xmark & \xmark & \cmark \\
%     \bottomrule
%     \end{tabular}
%     \caption{Comparison between existing task-oriented dialogue datasets and our DialogFlow dataset. 
%     % \textbf{Avg. Flow Steps} means the average number of steps of each dialogue flow.
%     }
%     \label{tab:dataset_compare}
% \end{table}


\begin{table}[t]
    \centering
    \small
    \begin{tabular}{@{}l@{\hskip 1mm}|@{\hskip 1mm}c@{\hskip 2mm}c@{\hskip 2mm}c@{}}
    \toprule
    & Task Plan? & Dialogue Flow? & Error Handling? \\
    \midrule
    MultiWOZ & \xmark & \xmark & \xmark  \\
    STAR & \xmark & \cmark & \xmark  \\
    ABCD & \cmark & \cmark & \xmark \\
    \midrule
    \dataset & \cmark & \cmark & \cmark \\
    \bottomrule
    \end{tabular}
    \caption{Comparison between existing task-oriented dialogue datasets and our \datasets dataset. }
    \label{tab:dataset_compare}
    % \vspace{2mm}
\end{table}

==> tab/dialog_prompt_ablation.tex <==
\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{p{0.93\linewidth}}
    \toprule
     \multicolumn{1}{l}{\textbf{Instruction and In-Context Example}} \\
     \midrule
     \textbf{Input}: Please generate a 6-turn conversation between a user and an agent for the task: "Explore the various car rental services offered". \\
    \midrule
     \textbf{Output}:  \\
     \underline{User}: Hi there! I'm planning a vacation, and I need to rent a car. Can you help me explore the various car rental services available?\\
    \underline{Agent}: Of course! I'd be happy to assist you in finding the best car rental service for your vacation. First off, may I know your destination and the dates you need the car?\\
    
    \underline{User}: I'll be traveling to Los Angeles, California, next month. I'll need the car from the 10th to the 20th.\\
    \underline{Agent}: Great! Los Angeles offers plenty of car rental options. Some popular ones include Hertz, Enterprise, Avis, Budget, and National Car Rental. Each has its unique features and benefits. Are you looking for any specific type of car or any particular requirements?\\
    
    \underline{User}: I'm looking for a comfortable sedan that can accommodate four people and has good fuel efficiency. Also, I'd prefer a rental service with unlimited mileage if possible.\\
    \underline{Agent}: Noted! For a comfortable sedan with good fuel efficiency, you can consider Hertz, as they offer a wide selection of vehicles. They usually have unlimited mileage options as well. Another good option is Enterprise, known for its excellent customer service and varied car choices. Would you like me to check their availability for your dates?\\
    
    \underline{User}: Yes, please check both Hertz and Enterprise for availability. Also, do they offer any loyalty programs or discounts?\\
    \underline{Agent}: Sure thing! I'll check the availability for your dates with both Hertz and Enterprise. Regarding loyalty programs, both companies do have reward programs where you can earn points for future rentals and enjoy various benefits. Hertz has the "Hertz Gold Plus Rewards," while Enterprise has the "Enterprise Plus" program. You can sign up for free and enjoy perks like priority service and faster reservations.\\
    
    \underline{User}: That sounds interesting! I'll definitely sign up for the loyalty programs. How about insurance options? Do they provide comprehensive coverage?\\
    \underline{Agent}:Yes, both Hertz and Enterprise offer insurance options to provide you with comprehensive coverage during your rental period. They typically offer Collision Damage Waiver (CDW), Liability Insurance, and Personal Accident Insurance. You can also opt for additional coverage if you prefer extra protection.\\
    
    \underline{User}: Perfect! I'll make sure to get the necessary insurance. One last question: do they have convenient pickup and drop-off locations near the airport?\\
    \underline{Agent}: Yes, both Hertz and Enterprise have multiple locations near Los Angeles International Airport (LAX) for easy pickup and drop-off. They also have branches throughout the city, so you can choose a location that's most convenient for you.\\

    \underline{User}: That's great news! Thank you so much for your help. I think I have a good idea now. I'll compare the prices and features before making a decision. \\
    \underline{Agent}: You're welcome! Take your time to compare, and if you have any more questions or need further assistance, feel free to reach out. Have a fantastic vacation in Los Angeles!
     \\ 
    \bottomrule
    \end{tabular}
    \caption{The prompt and in-context example for dialogue generation without task flow.
    \label{tab:dialog_prompt_ablation}}
\end{table*}
